The Transit Light Curve Project. VI. Three Transits of the Exoplanet TrES-2

Of the nearby transiting exoplanets that are amenable to detailed study, TrES-2 is both the most massive and has the largest impact parameter. We present z-band photometry of three transits of TrES-2. We improve upon the estimates of the planetary, stellar, and orbital parameters, in conjunction with the spectroscopic analysis of the host star by Sozzetti and co-workers. We find the planetary radius to be 1.222 +/- 0.038 R_Jup and the stellar radius to be 1.003 +/- 0.027 R_Sun. The quoted uncertainties include the systematic error due to the uncertainty in the stellar mass (0.980 +/- 0.062 M_Sun). The timings of the transits have an accuracy of 25s and are consistent with a uniform period, thus providing a baseline for future observations with the NASA Kepler satellite, whose field of view will include TrES-2.

==> tab1.tex <==
  2453989.63669 &          0.9992 &          0.0013 \\
  2453989.63943 &          1.0022 &          0.0013 \\
  2453989.64013 &          0.9994 &          0.0013 \\
  2453989.64058 &          0.9971 &          0.0013 \\
  2453989.64105 &          1.0002 &          0.0013 \\
  2453989.64150 &          0.9994 &          0.0013 \\
  2453989.64195 &          1.0000 &          0.0013 \\
  2453989.64240 &          1.0021 &          0.0013 \\
  2453989.64285 &          1.0000 &          0.0013 \\
  2453989.64330 &          0.9983 &          0.0013 \\
  2453989.64376 &          1.0018 &          0.0013 \\
  2453989.64422 &          0.9990 &          0.0013 \\
  2453989.64467 &          1.0030 &          0.0013 \\
  2453989.64512 &          1.0027 &          0.0013 \\
  2453989.64557 &          1.0006 &          0.0013 \\
  2453989.64602 &          1.0016 &          0.0013 \\
  2453989.64647 &          1.0001 &          0.0013 \\
  2453989.64693 &          1.0004 &          0.0013 \\
  2453989.64739 &          0.9987 &          0.0013 \\
  2453989.64784 &          1.0006 &          0.0013 \\
  2453989.64829 &          1.0022 &          0.0013 \\
  2453989.64874 &          1.0004 &          0.0013 \\
  2453989.64920 &          1.0011 &          0.0013 \\
  2453989.64965 &          1.0036 &          0.0013 \\
  2453989.65010 &          0.9970 &          0.0013 \\
  2453989.65101 &          1.0005 &          0.0013 \\
  2453989.65146 &          0.9984 &          0.0013 \\
  2453989.65191 &          0.9997 &          0.0013 \\
  2453989.65237 &          1.0010 &          0.0013 \\
  2453989.65282 &          1.0024 &          0.0013 \\
  2453989.65388 &          0.9981 &          0.0013 \\
  2453989.65433 &          1.0004 &          0.0013 \\
  2453989.65478 &          1.0007 &          0.0013 \\
  2453989.65524 &          1.0030 &          0.0013 \\
  2453989.65570 &          1.0019 &          0.0013 \\
  2453989.65615 &          1.0009 &          0.0013 \\
  2453989.65660 &          1.0005 &          0.0013 \\
  2453989.65705 &          1.0003 &          0.0013 \\
  2453989.65751 &          0.9995 &          0.0013 \\
  2453989.65796 &          1.0000 &          0.0013 \\
  2453989.65842 &          1.0011 &          0.0013 \\
  2453989.65887 &          0.9996 &          0.0013 \\
  2453989.65932 &          0.9990 &          0.0013 \\
  2453989.65977 &          0.9987 &          0.0013 \\
  2453989.66023 &          1.0005 &          0.0013 \\
  2453989.66068 &          1.0009 &          0.0013 \\
  2453989.66114 &          0.9997 &          0.0013 \\
  2453989.66159 &          1.0009 &          0.0013 \\
  2453989.66204 &          1.0017 &          0.0013 \\
  2453989.66249 &          0.9998 &          0.0013 \\
  2453989.66294 &          1.0017 &          0.0013 \\
  2453989.66340 &          1.0020 &          0.0013 \\
  2453989.66386 &          1.0005 &          0.0013 \\
  2453989.66431 &          0.9990 &          0.0013 \\
  2453989.66476 &          0.9982 &          0.0013 \\
  2453989.66521 &          0.9983 &          0.0013 \\
  2453989.66567 &          0.9988 &          0.0013 \\
  2453989.66612 &          0.9999 &          0.0013 \\
  2453989.66657 &          1.0004 &          0.0013 \\
  2453989.66703 &          0.9985 &          0.0013 \\
  2453989.66764 &          0.9971 &          0.0013 \\
  2453989.66810 &          0.9989 &          0.0013 \\
  2453989.66855 &          1.0019 &          0.0013 \\
  2453989.66901 &          1.0019 &          0.0013 \\
  2453989.66946 &          0.9991 &          0.0013 \\
  2453989.66991 &          1.0001 &          0.0013 \\
  2453989.67036 &          1.0034 &          0.0013 \\
  2453989.67081 &          1.0008 &          0.0013 \\
  2453989.67127 &          1.0014 &          0.0013 \\
  2453989.67173 &          0.9983 &          0.0013 \\
  2453989.67218 &          1.0007 &          0.0013 \\
  2453989.67263 &          0.9998 &          0.0013 \\
  2453989.67308 &          1.0015 &          0.0013 \\
  2453989.67354 &          0.9998 &          0.0013 \\
  2453989.67399 &          1.0002 &          0.0013 \\
  2453989.67445 &          1.0003 &          0.0013 \\
  2453989.67490 &          0.9980 &          0.0013 \\
  2453989.67535 &          0.9998 &          0.0013 \\
  2453989.67580 &          0.9988 &          0.0013 \\
  2453989.67625 &          0.9998 &          0.0013 \\
  2453989.67671 &          1.0007 &          0.0013 \\
  2453989.67717 &          1.0016 &          0.0013 \\
  2453989.67762 &          0.9976 &          0.0013 \\
  2453989.67852 &          1.0004 &          0.0013 \\
  2453989.67897 &          1.0009 &          0.0013 \\
  2453989.67943 &          0.9981 &          0.0013 \\
  2453989.67989 &          1.0003 &          0.0013 \\
  2453989.68034 &          0.9992 &          0.0013 \\
  2453989.68079 &          0.9999 &          0.0013 \\
  2453989.68132 &          1.0010 &          0.0013 \\
  2453989.68177 &          0.9991 &          0.0013 \\
  2453989.68223 &          0.9995 &          0.0013 \\
  2453989.68268 &          0.9978 &          0.0013 \\
  2453989.68313 &          1.0004 &          0.0013 \\
  2453989.68359 &          0.9988 &          0.0013 \\
  2453989.68404 &          1.0007 &          0.0013 \\
  2453989.68450 &          0.9995 &          0.0013 \\
  2453989.68495 &          1.0013 &          0.0013 \\
  2453989.68540 &          1.0001 &          0.0013 \\
  2453989.68585 &          1.0020 &          0.0013 \\
  2453989.68630 &          0.9999 &          0.0013 \\
  2453989.68676 &          1.0003 &          0.0013 \\
  2453989.68721 &          1.0014 &          0.0013 \\
  2453989.68767 &          1.0008 &          0.0013 \\
  2453989.68812 &          1.0011 &          0.0013 \\
  2453989.68857 &          0.9993 &          0.0013 \\
  2453989.68902 &          1.0001 &          0.0013 \\
  2453989.68947 &          0.9988 &          0.0013 \\
  2453989.68994 &          0.9993 &          0.0013 \\
  2453989.69039 &          1.0020 &          0.0013 \\
  2453989.69084 &          1.0010 &          0.0013 \\
  2453989.69129 &          0.9983 &          0.0013 \\
  2453989.69174 &          1.0012 &          0.0013 \\
  2453989.69219 &          1.0006 &          0.0013 \\
  2453989.69265 &          1.0013 &          0.0013 \\
  2453989.69311 &          1.0015 &          0.0013 \\
  2453989.69356 &          0.9993 &          0.0013 \\
  2453989.69401 &          1.0007 &          0.0013 \\
  2453989.69446 &          1.0005 &          0.0013 \\
  2453989.69491 &          1.0006 &          0.0013 \\
  2453989.69537 &          0.9983 &          0.0013 \\
  2453989.69583 &          1.0010 &          0.0013 \\
  2453989.69628 &          1.0023 &          0.0013 \\
  2453989.69673 &          1.0006 &          0.0013 \\
  2453989.69718 &          1.0009 &          0.0013 \\
  2453989.69763 &          0.9975 &          0.0013 \\
  2453989.69809 &          0.9996 &          0.0013 \\
  2453989.69855 &          1.0026 &          0.0013 \\
  2453989.69900 &          0.9993 &          0.0013 \\
  2453989.69945 &          1.0006 &          0.0013 \\
  2453989.69990 &          1.0007 &          0.0013 \\
  2453989.70035 &          1.0002 &          0.0013 \\
  2453989.70081 &          1.0007 &          0.0013 \\
  2453989.70127 &          0.9988 &          0.0013 \\
  2453989.70172 &          0.9997 &          0.0013 \\
  2453989.70217 &          0.9996 &          0.0013 \\
  2453989.70262 &          0.9974 &          0.0013 \\
  2453989.70307 &          1.0006 &          0.0013 \\
  2453989.70353 &          1.0002 &          0.0013 \\
  2453989.70399 &          0.9991 &          0.0013 \\
  2453989.70444 &          1.0003 &          0.0013 \\
  2453989.70489 &          1.0016 &          0.0013 \\
  2453989.70534 &          0.9982 &          0.0013 \\
  2453989.70624 &          1.0005 &          0.0013 \\
  2453989.70670 &          1.0001 &          0.0013 \\
  2453989.70716 &          0.9982 &          0.0013 \\
  2453989.70761 &          1.0005 &          0.0013 \\
  2453989.70806 &          1.0026 &          0.0013 \\
  2453989.70851 &          0.9995 &          0.0013 \\
  2453989.70896 &          1.0007 &          0.0013 \\
  2453989.70943 &          1.0001 &          0.0013 \\
  2453989.70988 &          1.0014 &          0.0013 \\
  2453989.71033 &          1.0005 &          0.0013 \\
  2453989.71078 &          1.0002 &          0.0013 \\
  2453989.71123 &          1.0007 &          0.0013 \\
  2453989.71168 &          0.9997 &          0.0013 \\
  2453989.71213 &          0.9991 &          0.0013 \\
  2453989.71260 &          0.9989 &          0.0013 \\
  2453989.71305 &          0.9990 &          0.0013 \\
  2453989.71350 &          0.9996 &          0.0013 \\
  2453989.71395 &          1.0004 &          0.0013 \\
  2453989.71485 &          0.9993 &          0.0013 \\
  2453989.71532 &          0.9982 &          0.0013 \\
  2453989.71577 &          1.0007 &          0.0013 \\
  2453989.71622 &          1.0025 &          0.0013 \\
  2453989.71667 &          0.9996 &          0.0013 \\
  2453989.71712 &          0.9970 &          0.0013 \\
  2453989.71757 &          1.0003 &          0.0013 \\
  2453989.71804 &          0.9963 &          0.0013 \\
  2453989.71849 &          0.9986 &          0.0013 \\
  2453989.71894 &          0.9996 &          0.0013 \\
  2453989.71939 &          0.9967 &          0.0013 \\
  2453989.71984 &          0.9998 &          0.0013 \\
  2453989.72029 &          0.9991 &          0.0013 \\
  2453989.72076 &          0.9977 &          0.0013 \\
  2453989.72121 &          0.9976 &          0.0013 \\
  2453989.72166 &          0.9947 &          0.0013 \\
  2453989.72211 &          0.9967 &          0.0013 \\
  2453989.72256 &          0.9956 &          0.0013 \\
  2453989.72301 &          0.9960 &          0.0013 \\
  2453989.72346 &          0.9948 &          0.0013 \\
  2453989.72393 &          0.9967 &          0.0013 \\
  2453989.72438 &          0.9928 &          0.0013 \\
  2453989.72483 &          0.9944 &          0.0013 \\
  2453989.72528 &          0.9949 &          0.0013 \\
  2453989.72573 &          0.9913 &          0.0013 \\
  2453989.72618 &          0.9940 &          0.0013 \\
  2453989.72665 &          0.9932 &          0.0013 \\
  2453989.72710 &          0.9941 &          0.0013 \\
  2453989.72755 &          0.9927 &          0.0013 \\
  2453989.72800 &          0.9932 &          0.0013 \\
  2453989.72845 &          0.9911 &          0.0013 \\
  2453989.72890 &          0.9918 &          0.0013 \\
  2453989.72937 &          0.9944 &          0.0013 \\
  2453989.72982 &          0.9909 &          0.0013 \\
  2453989.73027 &          0.9920 &          0.0013 \\
  2453989.73072 &          0.9910 &          0.0013 \\
  2453989.73117 &          0.9896 &          0.0013 \\
  2453989.73162 &          0.9910 &          0.0013 \\
  2453989.73209 &          0.9903 &          0.0013 \\
  2453989.73344 &          0.9901 &          0.0013 \\
  2453989.73389 &          0.9875 &          0.0013 \\
  2453989.73434 &          0.9892 &          0.0013 \\
  2453989.73479 &          0.9864 &          0.0013 \\
  2453989.73526 &          0.9872 &          0.0013 \\
  2453989.73628 &          0.9889 &          0.0013 \\
  2453989.73673 &          0.9862 &          0.0013 \\
  2453989.73764 &          0.9874 &          0.0013 \\
  2453989.73809 &          0.9850 &          0.0013 \\
  2453989.73855 &          0.9842 &          0.0013 \\
  2453989.73900 &          0.9868 &          0.0013 \\
  2453989.73945 &          0.9844 &          0.0013 \\
  2453989.73990 &          0.9864 &          0.0013 \\
  2453989.74036 &          0.9842 &          0.0013 \\
  2453989.74081 &          0.9865 &          0.0013 \\
  2453989.74126 &          0.9846 &          0.0013 \\
  2453989.74172 &          0.9846 &          0.0013 \\
  2453989.74217 &          0.9864 &          0.0013 \\
  2453989.74262 &          0.9850 &          0.0013 \\
  2453989.74308 &          0.9854 &          0.0013 \\
  2453989.74353 &          0.9874 &          0.0013 \\
  2453989.74398 &          0.9838 &          0.0013 \\
  2453989.74444 &          0.9836 &          0.0013 \\
  2453989.74489 &          0.9862 &          0.0013 \\
  2453989.74534 &          0.9853 &          0.0013 \\
  2453989.74580 &          0.9866 &          0.0013 \\
  2453989.74625 &          0.9853 &          0.0013 \\
  2453989.74670 &          0.9877 &          0.0014 \\
  2453989.74716 &          0.9859 &          0.0013 \\
  2453989.74761 &          0.9880 &          0.0013 \\
  2453989.74806 &          0.9855 &          0.0014 \\
  2453989.74851 &          0.9850 &          0.0013 \\
  2453989.74897 &          0.9841 &          0.0013 \\
  2453989.74942 &          0.9858 &          0.0014 \\
  2453989.74988 &          0.9859 &          0.0014 \\
  2453989.75033 &          0.9857 &          0.0014 \\
  2453989.75078 &          0.9846 &          0.0013 \\
  2453989.75123 &          0.9868 &          0.0014 \\
  2453989.75169 &          0.9855 &          0.0014 \\
  2453989.75214 &          0.9854 &          0.0014 \\
  2453989.75305 &          0.9856 &          0.0014 \\
  2453989.75350 &          0.9859 &          0.0014 \\
  2453989.75395 &          0.9852 &          0.0014 \\
  2453989.75441 &          0.9830 &          0.0014 \\
  2453989.75486 &          0.9844 &          0.0014 \\
  2453989.75532 &          0.9866 &          0.0014 \\
  2453989.75577 &          0.9845 &          0.0014 \\
  2453989.75622 &          0.9850 &          0.0014 \\
  2453989.75668 &          0.9862 &          0.0014 \\
  2453989.75713 &          0.9883 &          0.0014 \\
  2453989.75758 &          0.9855 &          0.0014 \\
  2453989.75803 &          0.9840 &          0.0014 \\
  2453989.75849 &          0.9834 &          0.0014 \\
  2453989.75894 &          0.9857 &          0.0014 \\
  2453989.75939 &          0.9848 &          0.0014 \\
  2453989.75985 &          0.9847 &          0.0014 \\
  2453989.76030 &          0.9876 &          0.0014 \\
  2453989.76076 &          0.9837 &          0.0014 \\
  2453989.76121 &          0.9862 &          0.0014 \\
  2453989.76166 &          0.9853 &          0.0014 \\
  2453989.76211 &          0.9851 &          0.0014 \\
  2453989.76256 &          0.9850 &          0.0014 \\
  2453989.76302 &          0.9841 &          0.0014 \\
  2453989.76347 &          0.9868 &          0.0014 \\
  2453989.76393 &          0.9827 &          0.0014 \\
  2453989.76438 &          0.9867 &          0.0014 \\
  2453989.76483 &          0.9854 &          0.0014 \\
  2453989.76528 &          0.9855 &          0.0014 \\
  2453989.76574 &          0.9862 &          0.0014 \\
  2453989.76620 &          0.9865 &          0.0014 \\
  2453989.76665 &          0.9881 &          0.0014 \\
  2453989.76710 &          0.9866 &          0.0014 \\
  2453989.76755 &          0.9854 &          0.0014 \\
  2453989.76800 &          0.9858 &          0.0014 \\
  2453989.76845 &          0.9879 &          0.0014 \\
  2453989.76891 &          0.9864 &          0.0014 \\
  2453989.76937 &          0.9887 &          0.0014 \\
  2453989.76982 &          0.9858 &          0.0014 \\
  2453989.77027 &          0.9905 &          0.0014 \\
  2453989.77072 &          0.9872 &          0.0014 \\
  2453989.77117 &          0.9908 &          0.0014 \\
  2453989.77163 &          0.9898 &          0.0014 \\
  2453989.77209 &          0.9861 &          0.0014 \\
  2453989.77254 &          0.9881 &          0.0014 \\
  2453989.77299 &          0.9873 &          0.0014 \\
  2453989.77344 &          0.9899 &          0.0014 \\
  2453989.77389 &          0.9895 &          0.0014 \\
  2453989.77434 &          0.9919 &          0.0014 \\
  2453989.77481 &          0.9921 &          0.0014 \\
  2453989.77526 &          0.9905 &          0.0014 \\
  2453989.77571 &          0.9904 &          0.0014 \\
  2453989.77616 &          0.9909 &          0.0014 \\
  2453989.77661 &          0.9926 &          0.0014 \\
  2453989.77706 &          0.9907 &          0.0014 \\
  2453989.77752 &          0.9934 &          0.0014 \\
  2453989.77798 &          0.9924 &          0.0014 \\
  2453989.77843 &          0.9917 &          0.0014 \\
  2453989.77888 &          0.9919 &          0.0014 \\
  2453989.77933 &          0.9924 &          0.0014 \\
  2453989.77978 &          0.9955 &          0.0014 \\
  2453989.78025 &          0.9931 &          0.0014 \\
  2453989.78070 &          0.9939 &          0.0014 \\
  2453989.78115 &          0.9949 &          0.0014 \\
  2453989.78160 &          0.9945 &          0.0014 \\
  2453989.78205 &          0.9951 &          0.0014 \\
  2453989.78250 &          0.9960 &          0.0014 \\
  2453989.78296 &          0.9989 &          0.0014 \\
  2453989.78342 &          0.9986 &          0.0014 \\
  2453989.78387 &          0.9982 &          0.0014 \\
  2453989.78432 &          0.9991 &          0.0014 \\
  2453989.78477 &          0.9932 &          0.0014 \\
  2453989.78522 &          0.9963 &          0.0014 \\
  2453989.78569 &          0.9984 &          0.0014 \\
  2453989.78614 &          0.9959 &          0.0014 \\
  2453989.78659 &          0.9984 &          0.0015 \\
  2453989.78704 &          1.0005 &          0.0014 \\
  2453989.78749 &          0.9978 &          0.0014 \\
  2453989.78795 &          0.9994 &          0.0014 \\
  2453989.78841 &          0.9979 &          0.0014 \\
  2453989.78886 &          0.9995 &          0.0014 \\
  2453989.78931 &          0.9984 &          0.0015 \\
  2453989.78976 &          0.9997 &          0.0015 \\
  2453989.79021 &          0.9995 &          0.0015 \\
  2453989.79275 &          1.0014 &          0.0015 \\
  2453989.79320 &          0.9978 &          0.0015 \\
  2453989.79365 &          0.9981 &          0.0015 \\
  2453989.79410 &          1.0004 &          0.0015 \\
  2453989.79455 &          0.9994 &          0.0015 \\
  2453989.79500 &          0.9994 &          0.0015 \\
  2453989.79546 &          0.9991 &          0.0015 \\
  2453989.79607 &          1.0016 &          0.0015 \\
  2453989.79652 &          0.9980 &          0.0015 \\
  2453989.79697 &          0.9998 &          0.0015 \\
  2453989.79743 &          0.9986 &          0.0015 \\
  2453989.79788 &          1.0016 &          0.0015 \\
  2453989.79833 &          1.0001 &          0.0015 \\
  2453989.79879 &          1.0014 &          0.0015 \\
  2453989.79924 &          0.9991 &          0.0015 \\
  2453989.79969 &          1.0009 &          0.0015 \\
  2453989.80015 &          0.9991 &          0.0015 \\
  2453989.80060 &          0.9990 &          0.0015 \\
  2453989.80106 &          1.0001 &          0.0015 \\
  2453989.80196 &          1.0027 &          0.0015 \\
  2453989.80242 &          1.0012 &          0.0015 \\
  2453989.80287 &          0.9996 &          0.0015 \\
  2453989.80332 &          0.9998 &          0.0015 \\
  2453989.80377 &          0.9996 &          0.0015 \\
  2453989.80423 &          1.0016 &          0.0015 \\
  2453989.80468 &          1.0029 &          0.0015 \\
  2453989.80514 &          0.9987 &          0.0015 \\
  2453989.80559 &          1.0008 &          0.0015 \\
  2453989.80604 &          1.0009 &          0.0015 \\
  2453989.80650 &          1.0014 &          0.0015 \\
  2453989.80695 &          0.9990 &          0.0015 \\
  2453989.80741 &          0.9994 &          0.0015 \\
  2453989.80786 &          1.0004 &          0.0015 \\
  2453989.80831 &          1.0013 &          0.0015 \\
  2453989.80876 &          1.0002 &          0.0015 \\
  2453989.80921 &          0.9993 &          0.0015 \\
  2453989.80967 &          1.0005 &          0.0015 \\
  2453989.81012 &          0.9979 &          0.0015 \\
  2453989.81058 &          0.9996 &          0.0015 \\
  2453989.81103 &          1.0021 &          0.0015 \\
  2453989.81148 &          0.9990 &          0.0016 \\
  2453989.81193 &          1.0014 &          0.0016 \\
  2453989.81239 &          0.9996 &          0.0016 \\
  2453989.81285 &          0.9984 &          0.0015 \\
  2453989.81330 &          0.9956 &          0.0016 \\
  2453989.81375 &          0.9994 &          0.0016 \\
  2453989.81420 &          1.0002 &          0.0016 \\
  2453989.81465 &          1.0023 &          0.0016 \\
  2453989.81511 &          1.0028 &          0.0016 \\
  2453989.81557 &          1.0008 &          0.0016 \\
  2453989.81602 &          1.0006 &          0.0016 \\
  2453989.81647 &          0.9994 &          0.0016 \\
  2453989.81692 &          0.9998 &          0.0016 \\
  2453989.81737 &          0.9995 &          0.0016 \\
  2453989.81782 &          1.0018 &          0.0016 \\
  2453989.81829 &          0.9983 &          0.0016 \\
  2453989.81874 &          1.0030 &          0.0016 \\
  2453989.81919 &          1.0007 &          0.0016 \\
  2453989.81964 &          0.9989 &          0.0016 \\
  2453989.82009 &          1.0006 &          0.0016 \\
  2453989.82055 &          1.0025 &          0.0016 \\
  2453989.82101 &          1.0003 &          0.0016 \\
  2453989.82146 &          0.9998 &          0.0016 \\
  2453989.82191 &          1.0004 &          0.0016 \\
  2453989.82236 &          1.0004 &          0.0016 \\
  2453989.82281 &          0.9993 &          0.0016 \\
  2453989.82326 &          0.9999 &          0.0016 \\
  2453989.82372 &          0.9972 &          0.0016 \\
  2453989.82418 &          0.9961 &          0.0016 \\
  2453989.82566 &          0.9990 &          0.0016 \\
  2453989.82611 &          1.0014 &          0.0016 \\
  2453989.82656 &          0.9985 &          0.0016 \\
  2453989.82701 &          1.0006 &          0.0016 \\
  2453989.82747 &          1.0009 &          0.0016 \\
  2453989.82793 &          1.0018 &          0.0016 \\
  2453989.82838 &          0.9985 &          0.0016 \\
  2453989.82883 &          0.9995 &          0.0016 \\
  2453989.82928 &          1.0028 &          0.0016 \\
  2453989.82974 &          0.9992 &          0.0017 \\
  2453989.83019 &          1.0025 &          0.0016 \\
  2453989.83064 &          0.9992 &          0.0017 \\
  2453989.83110 &          0.9994 &          0.0017 \\
  2453989.83155 &          1.0001 &          0.0017 \\
  2453989.83200 &          0.9999 &          0.0017 \\
  2453989.83245 &          1.0001 &          0.0017 \\
  2453989.83291 &          1.0027 &          0.0017 \\
  2453989.83336 &          0.9979 &          0.0017 \\
  2453989.83382 &          1.0027 &          0.0017 \\
  2453989.83427 &          1.0003 &          0.0017 \\
  2453989.83472 &          0.9980 &          0.0017 \\
  2453989.83518 &          1.0007 &          0.0017 \\
  2453989.83563 &          1.0005 &          0.0017 \\
  2453989.83608 &          1.0041 &          0.0017 \\
  2453989.83653 &          1.0022 &          0.0017 \\
  2453989.83699 &          1.0025 &          0.0017 \\
  2453989.83744 &          1.0014 &          0.0017 \\
  2453989.83789 &          1.0000 &          0.0017 \\
  2453989.84016 &          0.9984 &          0.0017 \\
  2453989.84107 &          0.9982 &          0.0017 \\
  2453989.84152 &          1.0018 &          0.0017 \\
  2453989.84197 &          0.9987 &          0.0018 \\
  2453989.84243 &          0.9988 &          0.0018 \\
  2453989.84288 &          1.0017 &          0.0017 \\
  2453989.84333 &          1.0018 &          0.0017 \\
  2453989.84379 &          1.0024 &          0.0018 \\
  2453989.84424 &          0.9991 &          0.0018 \\
  2453989.84469 &          0.9990 &          0.0018 \\
  2453989.84515 &          0.9995 &          0.0018 \\
  2453989.84560 &          1.0004 &          0.0018 \\
  2453989.84605 &          1.0001 &          0.0018 \\
  2453994.61930 &          0.9994 &          0.0014 \\
  2453994.62195 &          0.9992 &          0.0014 \\
  2453994.62243 &          1.0018 &          0.0014 \\
  2453994.62290 &          1.0003 &          0.0014 \\
  2453994.62338 &          0.9991 &          0.0014 \\
  2453994.62384 &          0.9989 &          0.0014 \\
  2453994.62434 &          0.9981 &          0.0014 \\
  2453994.62482 &          0.9989 &          0.0014 \\
  2453994.62530 &          1.0004 &          0.0014 \\
  2453994.62577 &          0.9997 &          0.0014 \\
  2453994.62627 &          1.0004 &          0.0014 \\
  2453994.62673 &          0.9991 &          0.0014 \\
  2453994.62723 &          0.9977 &          0.0014 \\
  2453994.62771 &          0.9997 &          0.0014 \\
  2453994.62818 &          1.0001 &          0.0014 \\
  2453994.62868 &          1.0009 &          0.0013 \\
  2453994.62918 &          0.9998 &          0.0014 \\
  2453994.62965 &          0.9994 &          0.0014 \\
  2453994.63013 &          0.9996 &          0.0014 \\
  2453994.63061 &          0.9994 &          0.0014 \\
  2453994.63111 &          0.9978 &          0.0014 \\
  2453994.63160 &          0.9996 &          0.0014 \\
  2453994.63209 &          0.9979 &          0.0014 \\
  2453994.63259 &          0.9991 &          0.0014 \\
  2453994.63307 &          0.9996 &          0.0014 \\
  2453994.63354 &          0.9989 &          0.0014 \\
  2453994.63403 &          0.9982 &          0.0014 \\
  2453994.63451 &          0.9994 &          0.0014 \\
  2453994.63500 &          1.0011 &          0.0013 \\
  2453994.63548 &          1.0019 &          0.0014 \\
  2453994.63597 &          1.0007 &          0.0013 \\
  2453994.63646 &          1.0014 &          0.0014 \\
  2453994.63694 &          0.9998 &          0.0013 \\
  2453994.63743 &          0.9997 &          0.0014 \\
  2453994.63790 &          1.0002 &          0.0014 \\
  2453994.63838 &          0.9993 &          0.0014 \\
  2453994.63888 &          0.9996 &          0.0013 \\
  2453994.63935 &          0.9988 &          0.0014 \\
  2453994.63985 &          0.9981 &          0.0014 \\
  2453994.64032 &          0.9987 &          0.0013 \\
  2453994.64082 &          0.9990 &          0.0014 \\
  2453994.64129 &          1.0023 &          0.0013 \\
  2453994.64178 &          0.9999 &          0.0013 \\
  2453994.64227 &          0.9995 &          0.0013 \\
  2453994.64275 &          1.0007 &          0.0013 \\
  2453994.64324 &          1.0010 &          0.0013 \\
  2453994.64372 &          0.9982 &          0.0013 \\
  2453994.64421 &          0.9992 &          0.0013 \\
  2453994.64470 &          1.0015 &          0.0013 \\
  2453994.64517 &          1.0004 &          0.0013 \\
  2453994.64565 &          1.0024 &          0.0013 \\
  2453994.64627 &          1.0032 &          0.0013 \\
  2453994.64676 &          1.0027 &          0.0013 \\
  2453994.64723 &          0.9994 &          0.0013 \\
  2453994.64769 &          0.9987 &          0.0013 \\
  2453994.64817 &          1.0006 &          0.0013 \\
  2453994.64866 &          1.0025 &          0.0013 \\
  2453994.64914 &          1.0004 &          0.0013 \\
  2453994.64965 &          1.0001 &          0.0013 \\
  2453994.65014 &          1.0013 &          0.0013 \\
  2453994.65063 &          1.0002 &          0.0013 \\
  2453994.65110 &          1.0008 &          0.0013 \\
  2453994.65160 &          0.9981 &          0.0014 \\
  2453994.65208 &          0.9992 &          0.0013 \\
  2453994.65257 &          0.9965 &          0.0013 \\
  2453994.65304 &          1.0006 &          0.0013 \\
  2453994.65354 &          1.0017 &          0.0013 \\
  2453994.65403 &          1.0010 &          0.0013 \\
  2453994.65449 &          1.0002 &          0.0013 \\
  2453994.65497 &          1.0006 &          0.0013 \\
  2453994.65547 &          0.9994 &          0.0013 \\
  2453994.65594 &          1.0015 &          0.0013 \\
  2453994.65643 &          0.9978 &          0.0013 \\
  2453994.65692 &          0.9990 &          0.0013 \\
  2453994.65739 &          1.0019 &          0.0013 \\
  2453994.65789 &          0.9998 &          0.0013 \\
  2453994.65838 &          1.0003 &          0.0013 \\
  2453994.65885 &          0.9955 &          0.0013 \\
  2453994.65934 &          0.9990 &          0.0013 \\
  2453994.65982 &          0.9950 &          0.0013 \\
  2453994.66030 &          0.9987 &          0.0013 \\
  2453994.66078 &          1.0001 &          0.0013 \\
  2453994.66127 &          0.9985 &          0.0014 \\
  2453994.66176 &          0.9982 &          0.0013 \\
  2453994.66224 &          0.9961 &          0.0014 \\
  2453994.66272 &          0.9948 &          0.0014 \\
  2453994.66320 &          0.9984 &          0.0013 \\
  2453994.66369 &          0.9976 &          0.0013 \\
  2453994.66416 &          0.9963 &          0.0014 \\
  2453994.66465 &          0.9966 &          0.0013 \\
  2453994.66514 &          0.9948 &          0.0014 \\
  2453994.66563 &          0.9944 &          0.0013 \\
  2453994.66611 &          0.9951 &          0.0014 \\
  2453994.66658 &          0.9926 &          0.0013 \\
  2453994.66706 &          0.9945 &          0.0013 \\
  2453994.66754 &          0.9941 &          0.0013 \\
  2453994.66801 &          0.9947 &          0.0013 \\
  2453994.66850 &          0.9942 &          0.0013 \\
  2453994.66898 &          0.9952 &          0.0013 \\
  2453994.66945 &          0.9927 &          0.0013 \\
  2453994.66993 &          0.9904 &          0.0014 \\
  2453994.67047 &          0.9910 &          0.0013 \\
  2453994.67096 &          0.9936 &          0.0013 \\
  2453994.67142 &          0.9903 &          0.0014 \\
  2453994.67194 &          0.9904 &          0.0014 \\
  2453994.67242 &          0.9918 &          0.0014 \\
  2453994.67291 &          0.9904 &          0.0014 \\
  2453994.67339 &          0.9892 &          0.0014 \\
  2453994.67387 &          0.9908 &          0.0013 \\
  2453994.67436 &          0.9884 &          0.0013 \\
  2453994.67485 &          0.9900 &          0.0014 \\
  2453994.67533 &          0.9893 &          0.0013 \\
  2453994.67582 &          0.9887 &          0.0014 \\
  2453994.67631 &          0.9907 &          0.0014 \\
  2453994.67678 &          0.9882 &          0.0014 \\
  2453994.67724 &          0.9882 &          0.0014 \\
  2453994.67773 &          0.9869 &          0.0014 \\
  2453994.67823 &          0.9858 &          0.0014 \\
  2453994.67870 &          0.9887 &          0.0014 \\
  2453994.67916 &          0.9861 &          0.0014 \\
  2453994.67965 &          0.9874 &          0.0014 \\
  2453994.68014 &          0.9871 &          0.0014 \\
  2453994.68061 &          0.9886 &          0.0014 \\
  2453994.68110 &          0.9864 &          0.0014 \\
  2453994.68158 &          0.9882 &          0.0014 \\
  2453994.68206 &          0.9880 &          0.0014 \\
  2453994.68253 &          0.9845 &          0.0014 \\
  2453994.68301 &          0.9854 &          0.0014 \\
  2453994.68349 &          0.9840 &          0.0014 \\
  2453994.68398 &          0.9862 &          0.0014 \\
  2453994.68446 &          0.9855 &          0.0014 \\
  2453994.68494 &          0.9859 &          0.0014 \\
  2453994.68540 &          0.9857 &          0.0014 \\
  2453994.68590 &          0.9853 &          0.0014 \\
  2453994.68637 &          0.9873 &          0.0014 \\
  2453994.68686 &          0.9838 &          0.0014 \\
  2453994.68736 &          0.9856 &          0.0014 \\
  2453994.68783 &          0.9840 &          0.0014 \\
  2453994.68832 &          0.9861 &          0.0014 \\
  2453994.68880 &          0.9849 &          0.0014 \\
  2453994.68929 &          0.9859 &          0.0014 \\
  2453994.68976 &          0.9859 &          0.0014 \\
  2453994.69024 &          0.9857 &          0.0014 \\
  2453994.69071 &          0.9846 &          0.0014 \\
  2453994.69120 &          0.9830 &          0.0014 \\
  2453994.69169 &          0.9853 &          0.0014 \\
  2453994.69217 &          0.9867 &          0.0014 \\
  2453994.69266 &          0.9865 &          0.0014 \\
  2453994.69314 &          0.9855 &          0.0014 \\
  2453994.69363 &          0.9868 &          0.0014 \\
  2453994.69413 &          0.9839 &          0.0014 \\
  2453994.69460 &          0.9841 &          0.0014 \\
  2453994.69508 &          0.9852 &          0.0014 \\
  2453994.69555 &          0.9866 &          0.0014 \\
  2453994.69605 &          0.9859 &          0.0014 \\
  2453994.69652 &          0.9851 &          0.0014 \\
  2453994.69702 &          0.9867 &          0.0014 \\
  2453994.69750 &          0.9854 &          0.0014 \\
  2453994.69798 &          0.9855 &          0.0014 \\
  2453994.69846 &          0.9849 &          0.0014 \\
  2453994.69894 &          0.9861 &          0.0014 \\
  2453994.69943 &          0.9857 &          0.0014 \\
  2453994.69990 &          0.9867 &          0.0014 \\
  2453994.70038 &          0.9869 &          0.0014 \\
  2453994.70086 &          0.9853 &          0.0014 \\
  2453994.70133 &          0.9862 &          0.0014 \\
  2453994.70181 &          0.9851 &          0.0014 \\
  2453994.70230 &          0.9880 &          0.0014 \\
  2453994.70279 &          0.9852 &          0.0014 \\
  2453994.70327 &          0.9841 &          0.0014 \\
  2453994.70375 &          0.9847 &          0.0014 \\
  2453994.70422 &          0.9866 &          0.0014 \\
  2453994.70469 &          0.9846 &          0.0014 \\
  2453994.70518 &          0.9866 &          0.0014 \\
  2453994.70568 &          0.9849 &          0.0014 \\
  2453994.70618 &          0.9891 &          0.0014 \\
  2453994.70665 &          0.9864 &          0.0014 \\
  2453994.70715 &          0.9902 &          0.0014 \\
  2453994.70763 &          0.9876 &          0.0014 \\
  2453994.70812 &          0.9884 &          0.0014 \\
  2453994.70861 &          0.9869 &          0.0014 \\
  2453994.70908 &          0.9866 &          0.0014 \\
  2453994.70956 &          0.9883 &          0.0014 \\
  2453994.71003 &          0.9864 &          0.0014 \\
  2453994.71050 &          0.9862 &          0.0014 \\
  2453994.71100 &          0.9862 &          0.0014 \\
  2453994.71149 &          0.9895 &          0.0014 \\
  2453994.71197 &          0.9880 &          0.0014 \\
  2453994.71247 &          0.9893 &          0.0014 \\
  2453994.71296 &          0.9886 &          0.0014 \\
  2453994.71344 &          0.9900 &          0.0014 \\
  2453994.71393 &          0.9881 &          0.0014 \\
  2453994.71442 &          0.9887 &          0.0014 \\
  2453994.71490 &          0.9914 &          0.0014 \\
  2453994.71539 &          0.9906 &          0.0014 \\
  2453994.71588 &          0.9921 &          0.0014 \\
  2453994.71636 &          0.9902 &          0.0014 \\
  2453994.71685 &          0.9899 &          0.0014 \\
  2453994.71732 &          0.9920 &          0.0014 \\
  2453994.71782 &          0.9923 &          0.0014 \\
  2453994.71829 &          0.9932 &          0.0014 \\
  2453994.71880 &          0.9943 &          0.0014 \\
  2453994.71929 &          0.9917 &          0.0014 \\
  2453994.71979 &          0.9938 &          0.0014 \\
  2453994.72026 &          0.9933 &          0.0014 \\
  2453994.72075 &          0.9931 &          0.0014 \\
  2453994.72123 &          0.9949 &          0.0014 \\
  2453994.72173 &          0.9942 &          0.0014 \\
  2453994.72221 &          0.9933 &          0.0014 \\
  2453994.72268 &          0.9950 &          0.0014 \\
  2453994.72317 &          0.9947 &          0.0014 \\
  2453994.72365 &          0.9954 &          0.0014 \\
  2453994.72415 &          0.9967 &          0.0014 \\
  2453994.72464 &          0.9980 &          0.0014 \\
  2453994.72511 &          0.9990 &          0.0014 \\
  2453994.72559 &          0.9990 &          0.0014 \\
  2453994.72606 &          0.9979 &          0.0014 \\
  2453994.72656 &          0.9985 &          0.0014 \\
  2453994.72703 &          0.9989 &          0.0014 \\
  2453994.72752 &          0.9970 &          0.0014 \\
  2453994.72800 &          0.9992 &          0.0014 \\
  2453994.72850 &          0.9987 &          0.0014 \\
  2453994.72899 &          1.0014 &          0.0014 \\
  2453994.72949 &          0.9975 &          0.0014 \\
  2453994.72995 &          1.0029 &          0.0014 \\
  2453994.73045 &          1.0003 &          0.0014 \\
  2453994.73093 &          1.0007 &          0.0014 \\
  2453994.73143 &          0.9989 &          0.0014 \\
  2453994.73189 &          1.0017 &          0.0014 \\
  2453994.73239 &          1.0032 &          0.0014 \\
  2453994.73287 &          0.9998 &          0.0014 \\
  2453994.73336 &          0.9997 &          0.0014 \\
  2453994.73384 &          0.9985 &          0.0014 \\
  2453994.73432 &          0.9998 &          0.0014 \\
  2453994.73480 &          1.0011 &          0.0014 \\
  2453994.73527 &          0.9988 &          0.0014 \\
  2453994.73576 &          0.9988 &          0.0014 \\
  2453994.73624 &          0.9983 &          0.0014 \\
  2453994.73672 &          1.0030 &          0.0014 \\
  2453994.73721 &          1.0009 &          0.0014 \\
  2453994.73768 &          0.9992 &          0.0014 \\
  2453994.73818 &          0.9993 &          0.0014 \\
  2453994.73866 &          0.9996 &          0.0014 \\
  2453994.73914 &          0.9978 &          0.0015 \\
  2453994.73961 &          0.9997 &          0.0014 \\
  2453994.74009 &          0.9983 &          0.0014 \\
  2453994.74055 &          0.9979 &          0.0014 \\
  2453994.74104 &          1.0004 &          0.0014 \\
  2453994.74152 &          0.9992 &          0.0014 \\
  2453994.74202 &          0.9985 &          0.0014 \\
  2453994.74251 &          0.9987 &          0.0014 \\
  2453994.74299 &          0.9992 &          0.0014 \\
  2453994.74348 &          1.0016 &          0.0015 \\
  2453994.74394 &          0.9974 &          0.0015 \\
  2453994.74445 &          0.9989 &          0.0015 \\
  2453994.74493 &          0.9997 &          0.0015 \\
  2453994.74541 &          0.9986 &          0.0015 \\
  2453994.74591 &          0.9984 &          0.0015 \\
  2453994.74640 &          1.0016 &          0.0015 \\
  2453994.74686 &          0.9987 &          0.0014 \\
  2453994.74735 &          0.9993 &          0.0014 \\
  2453994.74784 &          1.0019 &          0.0015 \\
  2453994.74830 &          0.9989 &          0.0015 \\
  2453994.74878 &          1.0008 &          0.0015 \\
  2453994.74925 &          0.9998 &          0.0015 \\
  2453994.74974 &          0.9990 &          0.0015 \\
  2453994.75023 &          1.0006 &          0.0015 \\
  2453994.75070 &          1.0029 &          0.0015 \\
  2453994.75118 &          1.0012 &          0.0015 \\
  2453994.75166 &          1.0001 &          0.0015 \\
  2453994.75214 &          1.0004 &          0.0015 \\
  2453994.75263 &          0.9959 &          0.0015 \\
  2453994.75312 &          0.9966 &          0.0015 \\
  2453994.75360 &          1.0001 &          0.0015 \\
  2453994.75408 &          1.0003 &          0.0015 \\
  2453994.75457 &          0.9995 &          0.0015 \\
  2453994.75506 &          0.9962 &          0.0015 \\
  2453994.75556 &          0.9988 &          0.0015 \\
  2453994.75604 &          1.0018 &          0.0015 \\
  2453994.75652 &          1.0017 &          0.0015 \\
  2453994.75699 &          1.0028 &          0.0015 \\
  2453994.75746 &          1.0007 &          0.0015 \\
  2453994.75795 &          1.0017 &          0.0015 \\
  2453994.75844 &          1.0001 &          0.0015 \\
  2453994.75892 &          1.0000 &          0.0015 \\
  2453994.75939 &          0.9958 &          0.0015 \\
  2453994.75989 &          0.9988 &          0.0015 \\
  2453994.76035 &          0.9988 &          0.0015 \\
  2453994.76083 &          1.0000 &          0.0015 \\
  2453994.76131 &          0.9963 &          0.0015 \\
  2453994.76179 &          1.0005 &          0.0015 \\
  2453994.76229 &          0.9991 &          0.0015 \\
  2453994.76277 &          1.0013 &          0.0015 \\
  2453994.76325 &          1.0007 &          0.0015 \\
  2453994.76371 &          0.9996 &          0.0015 \\
  2453994.76421 &          1.0002 &          0.0015 \\
  2453994.76468 &          1.0003 &          0.0015 \\
  2453994.76518 &          0.9992 &          0.0015 \\
  2453994.76565 &          1.0022 &          0.0015 \\
  2453994.76614 &          1.0023 &          0.0015 \\
  2453994.76664 &          1.0031 &          0.0015 \\
  2454041.56230 &          1.0012 &          0.0012 \\
  2454041.56279 &          0.9998 &          0.0012 \\
  2454041.56328 &          0.9981 &          0.0012 \\
  2454041.56375 &          0.9995 &          0.0012 \\
  2454041.56422 &          1.0006 &          0.0012 \\
  2454041.56471 &          1.0003 &          0.0012 \\
  2454041.56519 &          0.9999 &          0.0012 \\
  2454041.56567 &          0.9997 &          0.0012 \\
  2454041.56616 &          0.9997 &          0.0012 \\
  2454041.56666 &          1.0000 &          0.0012 \\
  2454041.56714 &          0.9995 &          0.0012 \\
  2454041.56763 &          1.0011 &          0.0012 \\
  2454041.56811 &          0.9995 &          0.0012 \\
  2454041.56860 &          0.9995 &          0.0012 \\
  2454041.56909 &          1.0022 &          0.0012 \\
  2454041.56957 &          0.9993 &          0.0012 \\
  2454041.57006 &          0.9992 &          0.0012 \\
  2454041.57053 &          0.9988 &          0.0012 \\
  2454041.57103 &          0.9996 &          0.0012 \\
  2454041.57152 &          1.0008 &          0.0012 \\
  2454041.57201 &          0.9985 &          0.0012 \\
  2454041.57250 &          0.9977 &          0.0012 \\
  2454041.57299 &          0.9999 &          0.0012 \\
  2454041.57347 &          1.0010 &          0.0012 \\
  2454041.57444 &          1.0004 &          0.0012 \\
  2454041.57493 &          1.0004 &          0.0012 \\
  2454041.57540 &          1.0001 &          0.0012 \\
  2454041.57588 &          0.9993 &          0.0012 \\
  2454041.57637 &          0.9975 &          0.0012 \\
  2454041.57685 &          0.9998 &          0.0012 \\
  2454041.57734 &          0.9985 &          0.0012 \\
  2454041.57781 &          0.9975 &          0.0012 \\
  2454041.57829 &          0.9992 &          0.0012 \\
  2454041.57877 &          0.9995 &          0.0012 \\
  2454041.57926 &          1.0000 &          0.0012 \\
  2454041.57975 &          0.9992 &          0.0012 \\
  2454041.58022 &          1.0023 &          0.0012 \\
  2454041.58072 &          0.9971 &          0.0012 \\
  2454041.58120 &          0.9983 &          0.0012 \\
  2454041.58168 &          1.0007 &          0.0012 \\
  2454041.58216 &          0.9994 &          0.0012 \\
  2454041.58264 &          1.0000 &          0.0012 \\
  2454041.58312 &          1.0010 &          0.0012 \\
  2454041.58361 &          0.9987 &          0.0012 \\
  2454041.58410 &          0.9992 &          0.0012 \\
  2454041.58459 &          1.0006 &          0.0012 \\
  2454041.58508 &          1.0008 &          0.0012 \\
  2454041.58557 &          0.9977 &          0.0012 \\
  2454041.58605 &          1.0018 &          0.0012 \\
  2454041.58659 &          0.9971 &          0.0012 \\
  2454041.58707 &          1.0006 &          0.0012 \\
  2454041.58757 &          0.9995 &          0.0012 \\
  2454041.58804 &          1.0002 &          0.0012 \\
  2454041.58853 &          1.0002 &          0.0012 \\
  2454041.58902 &          1.0035 &          0.0012 \\
  2454041.58951 &          0.9986 &          0.0012 \\
  2454041.59000 &          1.0020 &          0.0013 \\
  2454041.59047 &          1.0012 &          0.0012 \\
  2454041.59097 &          1.0009 &          0.0012 \\
  2454041.59146 &          1.0012 &          0.0012 \\
  2454041.59193 &          1.0016 &          0.0012 \\
  2454041.59242 &          0.9973 &          0.0012 \\
  2454041.59289 &          1.0016 &          0.0012 \\
  2454041.59337 &          0.9981 &          0.0012 \\
  2454041.59384 &          0.9997 &          0.0012 \\
  2454041.59433 &          0.9989 &          0.0012 \\
  2454041.59483 &          0.9991 &          0.0012 \\
  2454041.59529 &          1.0006 &          0.0012 \\
  2454041.59577 &          0.9979 &          0.0012 \\
  2454041.59626 &          1.0009 &          0.0012 \\
  2454041.59676 &          0.9999 &          0.0012 \\
  2454041.59724 &          1.0019 &          0.0012 \\
  2454041.59773 &          1.0020 &          0.0012 \\
  2454041.59822 &          0.9993 &          0.0012 \\
  2454041.59871 &          1.0004 &          0.0012 \\
  2454041.59921 &          1.0011 &          0.0012 \\
  2454041.59969 &          0.9993 &          0.0012 \\
  2454041.60018 &          1.0011 &          0.0012 \\
  2454041.60065 &          0.9965 &          0.0012 \\
  2454041.60115 &          1.0003 &          0.0012 \\
  2454041.60165 &          0.9975 &          0.0012 \\
  2454041.60213 &          1.0000 &          0.0012 \\
  2454041.60263 &          0.9998 &          0.0012 \\
  2454041.60310 &          0.9986 &          0.0012 \\
  2454041.60359 &          0.9987 &          0.0012 \\
  2454041.60407 &          0.9954 &          0.0012 \\
  2454041.60456 &          0.9973 &          0.0012 \\
  2454041.60505 &          0.9959 &          0.0012 \\
  2454041.60554 &          0.9975 &          0.0012 \\
  2454041.60603 &          0.9962 &          0.0013 \\
  2454041.60653 &          0.9936 &          0.0013 \\
  2454041.60699 &          0.9945 &          0.0012 \\
  2454041.60747 &          0.9961 &          0.0013 \\
  2454041.60796 &          0.9955 &          0.0012 \\
  2454041.60845 &          0.9942 &          0.0013 \\
  2454041.60894 &          0.9932 &          0.0013 \\
  2454041.60942 &          0.9910 &          0.0013 \\
  2454041.60991 &          0.9923 &          0.0013 \\
  2454041.61039 &          0.9923 &          0.0013 \\
  2454041.61091 &          0.9934 &          0.0013 \\
  2454041.61139 &          0.9932 &          0.0013 \\
  2454041.61187 &          0.9901 &          0.0013 \\
  2454041.61237 &          0.9924 &          0.0013 \\
  2454041.61283 &          0.9919 &          0.0013 \\
  2454041.61332 &          0.9899 &          0.0013 \\
  2454041.61382 &          0.9916 &          0.0013 \\
  2454041.61429 &          0.9912 &          0.0013 \\
  2454041.61479 &          0.9907 &          0.0013 \\
  2454041.61525 &          0.9899 &          0.0013 \\
  2454041.61575 &          0.9885 &          0.0013 \\
  2454041.61624 &          0.9903 &          0.0013 \\
  2454041.61671 &          0.9909 &          0.0013 \\
  2454041.61720 &          0.9902 &          0.0013 \\
  2454041.61768 &          0.9883 &          0.0013 \\
  2454041.61818 &          0.9878 &          0.0013 \\
  2454041.61866 &          0.9873 &          0.0013 \\
  2454041.61914 &          0.9868 &          0.0013 \\
  2454041.61963 &          0.9852 &          0.0013 \\
  2454041.62009 &          0.9893 &          0.0013 \\
  2454041.62059 &          0.9867 &          0.0013 \\
  2454041.62107 &          0.9868 &          0.0013 \\
  2454041.62155 &          0.9869 &          0.0013 \\
  2454041.62202 &          0.9892 &          0.0013 \\
  2454041.62251 &          0.9869 &          0.0013 \\
  2454041.62302 &          0.9866 &          0.0013 \\
  2454041.62352 &          0.9862 &          0.0013 \\
  2454041.62399 &          0.9872 &          0.0013 \\
  2454041.62447 &          0.9887 &          0.0013 \\
  2454041.62493 &          0.9865 &          0.0013 \\
  2454041.62542 &          0.9862 &          0.0013 \\
  2454041.62592 &          0.9882 &          0.0013 \\
  2454041.62639 &          0.9860 &          0.0013 \\
  2454041.62688 &          0.9856 &          0.0013 \\
  2454041.62738 &          0.9884 &          0.0013 \\
  2454041.62787 &          0.9888 &          0.0013 \\
  2454041.62835 &          0.9872 &          0.0013 \\
  2454041.62884 &          0.9870 &          0.0013 \\
  2454041.62932 &          0.9870 &          0.0013 \\
  2454041.62980 &          0.9856 &          0.0013 \\
  2454041.63029 &          0.9855 &          0.0013 \\
  2454041.63079 &          0.9848 &          0.0013 \\
  2454041.63126 &          0.9864 &          0.0013 \\
  2454041.63176 &          0.9872 &          0.0013 \\
  2454041.63224 &          0.9860 &          0.0013 \\
  2454041.63272 &          0.9854 &          0.0013 \\
  2454041.63320 &          0.9847 &          0.0013 \\
  2454041.63370 &          0.9857 &          0.0013 \\
  2454041.63419 &          0.9847 &          0.0013 \\
  2454041.63467 &          0.9849 &          0.0013 \\
  2454041.63515 &          0.9853 &          0.0013 \\
  2454041.63565 &          0.9841 &          0.0013 \\
  2454041.63613 &          0.9853 &          0.0013 \\
  2454041.63662 &          0.9853 &          0.0013 \\
  2454041.63710 &          0.9871 &          0.0013 \\
  2454041.63760 &          0.9877 &          0.0013 \\
  2454041.63809 &          0.9854 &          0.0013 \\
  2454041.63857 &          0.9858 &          0.0013 \\
  2454041.63906 &          0.9833 &          0.0013 \\
  2454041.63955 &          0.9841 &          0.0013 \\
  2454041.64004 &          0.9864 &          0.0013 \\
  2454041.64054 &          0.9852 &          0.0013 \\
  2454041.64103 &          0.9862 &          0.0013 \\
  2454041.64151 &          0.9861 &          0.0013 \\
  2454041.64200 &          0.9869 &          0.0013 \\
  2454041.64249 &          0.9852 &          0.0013 \\
  2454041.64296 &          0.9831 &          0.0013 \\
  2454041.64346 &          0.9877 &          0.0013 \\
  2454041.64394 &          0.9871 &          0.0013 \\
  2454041.64443 &          0.9877 &          0.0013 \\
  2454041.64493 &          0.9857 &          0.0013 \\
  2454041.64541 &          0.9857 &          0.0013 \\
  2454041.64590 &          0.9867 &          0.0013 \\
  2454041.64640 &          0.9879 &          0.0013 \\
  2454041.64686 &          0.9866 &          0.0013 \\
  2454041.64740 &          0.9869 &          0.0013 \\
  2454041.64788 &          0.9860 &          0.0014 \\
  2454041.64838 &          0.9851 &          0.0013 \\
  2454041.64886 &          0.9843 &          0.0013 \\
  2454041.64936 &          0.9868 &          0.0013 \\
  2454041.64985 &          0.9900 &          0.0014 \\
  2454041.65033 &          0.9857 &          0.0013 \\
  2454041.65082 &          0.9870 &          0.0013 \\
  2454041.65130 &          0.9865 &          0.0013 \\
  2454041.65180 &          0.9886 &          0.0013 \\
  2454041.65228 &          0.9866 &          0.0013 \\
  2454041.65276 &          0.9894 &          0.0013 \\
  2454041.65326 &          0.9882 &          0.0013 \\
  2454041.65372 &          0.9902 &          0.0013 \\
  2454041.65422 &          0.9909 &          0.0013 \\
  2454041.65471 &          0.9908 &          0.0013 \\
  2454041.65521 &          0.9900 &          0.0013 \\
  2454041.65568 &          0.9908 &          0.0013 \\
  2454041.65614 &          0.9897 &          0.0013 \\
  2454041.65663 &          0.9889 &          0.0013 \\
  2454041.65713 &          0.9915 &          0.0013 \\
  2454041.65760 &          0.9913 &          0.0013 \\
  2454041.65809 &          0.9904 &          0.0013 \\
  2454041.65857 &          0.9888 &          0.0013 \\
  2454041.65906 &          0.9915 &          0.0013 \\
  2454041.65957 &          0.9910 &          0.0013 \\
  2454041.66005 &          0.9927 &          0.0013 \\
  2454041.66052 &          0.9925 &          0.0013 \\
  2454041.66102 &          0.9923 &          0.0014 \\
  2454041.66150 &          0.9922 &          0.0014 \\
  2454041.66199 &          0.9914 &          0.0014 \\
  2454041.66246 &          0.9963 &          0.0014 \\
  2454041.66296 &          0.9950 &          0.0014 \\
  2454041.66343 &          0.9950 &          0.0014 \\
  2454041.66392 &          0.9937 &          0.0014 \\
  2454041.66441 &          0.9933 &          0.0014 \\
  2454041.66490 &          0.9967 &          0.0014 \\
  2454041.66539 &          0.9949 &          0.0014 \\
  2454041.66589 &          0.9956 &          0.0014 \\
  2454041.66636 &          0.9943 &          0.0014 \\
  2454041.66687 &          0.9982 &          0.0014 \\
  2454041.66736 &          0.9956 &          0.0014 \\
  2454041.66786 &          0.9972 &          0.0014 \\
  2454041.66834 &          1.0008 &          0.0014 \\
  2454041.66883 &          0.9962 &          0.0014 \\
  2454041.66933 &          0.9981 &          0.0014 \\
  2454041.66979 &          0.9979 &          0.0014 \\
  2454041.67029 &          0.9979 &          0.0014 \\
  2454041.67076 &          0.9982 &          0.0014 \\
  2454041.67123 &          0.9995 &          0.0014 \\
  2454041.67173 &          0.9980 &          0.0014 \\
  2454041.67221 &          0.9955 &          0.0014 \\
  2454041.67270 &          0.9997 &          0.0014 \\
  2454041.67318 &          1.0014 &          0.0014 \\
  2454041.67365 &          0.9999 &          0.0014 \\
  2454041.67414 &          1.0008 &          0.0014 \\
  2454041.67460 &          1.0015 &          0.0014 \\
  2454041.67509 &          1.0003 &          0.0014 \\
  2454041.67556 &          0.9997 &          0.0014 \\
  2454041.67606 &          1.0006 &          0.0014 \\
  2454041.67655 &          0.9997 &          0.0014 \\
  2454041.67704 &          0.9991 &          0.0014 \\
  2454041.67752 &          0.9987 &          0.0014 \\
  2454041.67799 &          0.9999 &          0.0014 \\
  2454041.67848 &          0.9980 &          0.0014 \\
  2454041.67898 &          1.0006 &          0.0014 \\
  2454041.67948 &          1.0004 &          0.0014 \\
  2454041.67996 &          1.0008 &          0.0014 \\
  2454041.68045 &          1.0011 &          0.0014 \\
  2454041.68093 &          1.0007 &          0.0014 \\
  2454041.68142 &          0.9974 &          0.0014 \\
  2454041.68191 &          0.9992 &          0.0014 \\
  2454041.68239 &          1.0000 &          0.0014 \\
  2454041.68288 &          0.9997 &          0.0014 \\
  2454041.68335 &          1.0007 &          0.0014 \\
  2454041.68385 &          1.0004 &          0.0014 \\
  2454041.68434 &          0.9985 &          0.0014 \\
  2454041.68482 &          1.0006 &          0.0014 \\
  2454041.68531 &          0.9986 &          0.0014 \\
  2454041.68581 &          0.9991 &          0.0014 \\
  2454041.68627 &          0.9981 &          0.0014 \\
  2454041.68677 &          1.0003 &          0.0014 \\
  2454041.68724 &          1.0022 &          0.0014 \\
  2454041.68774 &          1.0019 &          0.0014 \\
  2454041.68824 &          0.9991 &          0.0015 \\
  2454041.68872 &          1.0019 &          0.0014 \\
  2454041.68920 &          0.9974 &          0.0014 \\
  2454041.68968 &          1.0003 &          0.0015 \\
  2454041.69017 &          0.9999 &          0.0015 \\
  2454041.69066 &          1.0005 &          0.0015 \\
  2454041.69113 &          0.9975 &          0.0015 \\
  2454041.69163 &          0.9998 &          0.0015 \\
  2454041.69211 &          1.0011 &          0.0015 \\
  2454041.69260 &          0.9985 &          0.0015 \\
  2454041.69309 &          1.0012 &          0.0015 \\
  2454041.69357 &          1.0006 &          0.0015 \\
  2454041.69407 &          1.0000 &          0.0015 \\
  2454041.69453 &          1.0004 &          0.0015 \\
  2454041.69503 &          0.9994 &          0.0015 \\
  2454041.69552 &          0.9992 &          0.0015 \\
  2454041.69603 &          1.0002 &          0.0015 \\
  2454041.69651 &          0.9975 &          0.0015 \\
  2454041.69700 &          0.9996 &          0.0015 \\
  2454041.69748 &          0.9996 &          0.0015 \\
  2454041.69798 &          1.0004 &          0.0015 \\
  2454041.69846 &          1.0013 &          0.0015 \\
  2454041.69894 &          1.0003 &          0.0015 \\
  2454041.69942 &          0.9993 &          0.0015 \\
  2454041.69990 &          1.0016 &          0.0015 \\
  2454041.70038 &          1.0012 &          0.0015 \\
  2454041.70085 &          1.0022 &          0.0016 \\
  2454041.70135 &          0.9986 &          0.0016 \\
  2454041.70184 &          0.9969 &          0.0016 \\
  2454041.70231 &          1.0004 &          0.0016 \\
  2454041.70279 &          1.0003 &          0.0016 \\
  2454041.70327 &          1.0014 &          0.0016 \\
  2454041.70376 &          1.0007 &          0.0016 \\
  2454041.70426 &          0.9992 &          0.0016 \\
  2454041.70473 &          0.9993 &          0.0016 \\
  2454041.70522 &          1.0000 &          0.0016 \\
  2454041.70570 &          1.0007 &          0.0016 \\
  2454041.70619 &          0.9992 &          0.0016 \\
  2454041.70667 &          0.9996 &          0.0016 \\
  2454041.70716 &          1.0000 &          0.0016 \\
  2454041.70766 &          0.9983 &          0.0016 \\

